Topological Descriptors for Parkinson's Disease Classification and Regression Analysis

At present, the vast majority of human subjects with neurological disease are still diagnosed through in-person assessments and qualitative analysis of patient data. In this paper, we propose to use Topological Data Analysis (TDA) together with machine learning tools to automate the process of Parkinson's disease classification and severity assessment. An automated, stable, and accurate method to evaluate Parkinson's would be significant in streamlining diagnoses of patients and providing families more time for corrective measures. We propose a methodology which incorporates TDA into analyzing Parkinson's disease postural shifts data through the representation of persistence images. Studying the topology of a system has proven to be invariant to small changes in data and has been shown to perform well in discrimination tasks. The contributions of the paper are twofold. We propose a method to 1) classify healthy patients from those afflicted by disease and 2) diagnose the severity of disease. We explore the use of the proposed method in an application involving a Parkinson's disease dataset comprised of healthy-elderly, healthy-young and Parkinson's disease patients. Our code is available at https://github.com/itsmeafra/Sublevel-Set-TDA.

==> 03_Dataset.tex <==
\vspace{-0.05in}
\section{Dataset}\label{dataset}
\vspace{-0.05in}

%describes Dr. Krishnamurthi's dataset for the knowledge of paper readers?
%dont know if this section is necessary

%different groups - old young pd
%different columns - x, y, z, fx, fy, fz, mx, my, mz
%number of subjects in each group
%number of trials per subject
%description of how data was taken
%type of data

%MENTION IN THE EXPERIMENT SECTION BRIEFLY INSTEAD OF HAVING AN ENTIRE SECTION FOR THIS (and then reference a separate paper to direct readers to more info on how the data is collected)

%The dataset used for analysis of our proposed method is the same as that used for two studies before it (anirudhs and the one anirudh references). The dataset contains patients categorized into three separate groups - old, young, and PD (Parkinson's disease). For each subject in the dataset, multiple samples of time series pressure point data was taken. For healthy patients - i.e. those patients that fall into the young and old categories - 5 trials were taken, while for those with Parkinson's disease 3 trials were taken. To obtain these samples, patients were asked to stand still, with their hands to their sides, on a pressure point platform. They then were able to see a cursor on a screen that represented their real time center of mass. At the start of each trial, the cursor began at a base position. A target was then shown to the subject and the subject was instructed to reach toward the target. The subjects aim was thus to move their cursor from the base to the new target and maintain this position for 2 seconds. There were 5 different targets from which subjects were instructed to go to and from including 0, 45, 90, 135, and 180 degree angles. This resulted in 10 reaches per subject trial (again to and from each target). The order in which these targets would appear was randomized. 

==> 07_References.tex <==
\vspace{-0.05in}
\section{References}\label{references}
\vspace{-0.05in}

[1] Anirudh Attractor Shape Descriptors
\newline [2] Anirudh Multi-Scale Attractor Shape Descriptors
\newline [3] Anirudh PI-Net Paper
\newline [4] Short Survey of Topological Data Analysis
\newline [5] Persistence Based Structural Recognition
\newline [6] Short Survey of Topological Data Analysis in Time Series and Signals Analysis
\newline [7] Perturbation Robust Representations of \newline Topological Persistence Diagrams
\newline [8] World Health Organization, Neurological Disorders Public Health Challenges (2006). June 2018
\newline [9] Paper with Statistics on Prevalence of PD
\newline [10] A survey of Parkinson's disease patients: most bothersome symptoms and coping preferences.
\newline [11] Deterioration of Parkinson’s disease during hospitalization: survey of 684 patients (Canada?)
\newline [12] A Step Towards the Automated Diagnosis of Parkinson’s Disease: Analyzing Handwriting Movements
\newline [13] Fully Automated Assessment of the Severity of Parkinson’s Disease from Speech
\newline [14] A deep learning approach for Parkinson’s disease diagnosis from EEG signals
\newline [15] Automatic recognition of gait-related health problems in the elderly using machine learning
\newline [16] Machine learning on brain MRI data for differential diagnosis of Parkinson’s disease and Progressive Supranuclear Palsy
\newline [17] Persistence Images: A Stable Vector Representation of Persistent Homology
\newline [18] Mathematical Tools for Shape Analysis and Description
\newline [19] Machine learning for Medical Diagnoses: history, state of the art and perspective
